Towards Safe Automated Refactoring of Imperative Deep Learning Programs to Graph Execution

Efficiency is essential to support responsiveness w.r.t. ever-growing datasets, especially for Deep Learning (DL) systems. DL frameworks have traditionally embraced deferred execution-style DL code -- supporting symbolic, graph-based Deep Neural Network (DNN) computation. While scalable, such development tends to produce code that is error-prone, non-intuitive, and difficult to debug. Consequently, more natural, less error-prone imperative DL frameworks encouraging eager execution have emerged at the expense of run-time performance. Though hybrid approaches aim for the "best of both worlds," using them effectively requires subtle considerations to make code amenable to safe, accurate, and efficient graph execution -- avoiding performance bottlenecks and semantically inequivalent results. We present our ongoing work on an automated refactoring approach that assists developers in specifying whether and how their otherwise eagerly-executed imperative DL code could be reliably and efficiently executed as graphs at run-time in a semantics-preserving fashion. The approach, based on a novel tensor analysis specifically for imperative DL code, consists of refactoring preconditions for automatically determining when it is safe and potentially advantageous to migrate imperative DL code to graph execution and modifying decorator parameters or eagerly executing code already running as graphs. The approach is being implemented as a PyDev Eclipse IDE plug-in and uses the WALA Ariadne analysis framework. We discuss our ongoing work towards optimizing imperative DL code to its full potential.

==> Makefile <==
PAPER=paper
all:
	latexmk -pdf -shell-escape $(PAPER)
automated:
	latexmk -pdf -shell-escape -interaction=nonstopmode $(PAPER)
continuous:
	latexmk -pdf -pvc -shell-escape $(PAPER)
preview: all
	gio open $(PAPER).pdf
clean:
	latexmk -C $(PAPER)
	rm -rf _minted-*
	rm -f *.aux *.log *.bbl *.blg *.dvi *.synctex.gz *.out *.fdb_latexmk \
		*.fls *.nav *.toc *.snm *.spl *.vtc *.pyg *.vrb *.bcf *.run.xml *.tdo \
		*-blx.bib
	rm -rf $(PAPER)
test: automated
	chktex -xH -n 6 $(PAPER).tex 2> /dev/null | tee lint.out
	test ! -s lint.out
	! grep -Hn ' $$' *.tex # check for trailing whitespace.
	! grep -Hni 'undefined references' $(PAPER).log # check for undefined references.
	! grep -Hni 'multiply defined' $(PAPER).log # check for multiply defined entities.
	# ! grep -n "LaTeX Warning" $(PAPER).log
html: all
	rm -rf $(PAPER)/
	latex2html -split 0 $(PAPER)
	gio open $(PAPER)/index.html
TODO:
	pandoc -s --metadata title="TODOs" TODO.md -o TODO.html
preview-TODO: TODO
	gio open TODO.html
install-arxiv-latex-cleaner:
	pip install arxiv-latex-cleaner
arXiv:
	scripts/prep_arXiv.sh


==> eval.tex <==
\section{Evaluation}\label{sec:eval}

\subsection{Implementation}\label{sec:impl}

An important advantage of building our plug-in atop of PyDev is its fast indexing feature, which makes looking up program entities, e.g., FQN lookup, extremely fast.

Although \citetitle{Dolby2018} has Python parsing capabilities, we integrated it with PyDev due to PyDev's excellent and long-lived refactoring support for Python, including refactoring preview pane, element GUI selection, and refactoring undo history. In other words, \citetitle{Dolby2018}, like WALA, is an program \emph{analysis} framework and thus does not have AST manipulation capabilities that have been traditionally found in IDEs. PyDev, being an IDE plug-in, can \emph{transform} Python ASTs. An alternative would be to use the analysis results from \citetitle{Dobly2018} to guide refactoring recommendations that are then sent to the IDE via the Language Server Protocol (LSP)~\cite{MicrosoftCorporation2022}. Then, an IDE receiving the LSP messages would be responsible for executing the refactoring. However, support for refactoring in LSP is pending~\cite{Istria2021,Tuppeny2023}.

\subsection{Subject Preparation}

Because our plug-in resolves FQNs, we need the subject project dependencies to analyze them. Thus, before running our experiments, we need to run an installation script. Unfortunately, Python has several ways to install project dependencies (e.g., \ti{requirements.txt}, \ti{distutils}, \ti{setup.py}), and some project may not include installation scripts. If \ti{requirements.txt}---a common Python idiom to list dependencies along with their versions---is not found, we use \ti{pireqs} to generate one. The \ti{pireqs} tool is a standard tool for Python that analyzes import statements in a project and generates an appropriate \ti{requirements.txt} file. We then use \ti{pip}, the Python package manager, to install all of the found dependencies. Otherwise, various import statements in the subject project source code may not be resolved by our plug-in. The situation is analogous to running a static analysis/refactoring tool to, e.g., C++, Java, code that does not originally compile and expecting sound results. At least in the dynamic case, requiring imports to be resolved gives us a bit more information to analyze the code base. And, when analyzing code written in dynamic languages, since static information is so sparse, and piece of information can prove useful.

In our test suite, we check if the code runs before and after the refactoring by adding a \pyi{__main__} function and ensuring that we cover all of the Python code lines in the test file. Moreover, each test case has its own \ti{requirements.txt} file, and the first step in running a test case is invoking the package manager, \pyi{pip3}, with that file.


==> latexdiff.tex <==
#!/bin/bash
PAPER="paper"
set -vx
latexdiff-git --force -d -r $1 *.tex *.bbl
cd diff$1
ln -s ../Makefile
ln -s ../paper.bib
ln -s ../graphics
make preview
cd ..


==> related.tex <==
\section{Related Work}\label{sec:related}

\cite{Cao2022} %
\cite{Baker2022} %


==> threats.tex <==
\section{Threads to Validity}\label{sec:threats}

The work will be in designing recommendation systems, so software developers will still be in charge of making the final decisions on the recommended transformations.

Currently, we do not process iPython Notebooks. Some of the projects we encountered during the evaluation include such notebooks in their repositories. It is possible that hybridization opportunities exist in these notebooks, and our approach will miss them. However, we found a common pattern to be that examples of how to use the projects are found in this notebooks as opposed to the core functionality of the project. It is also possible that entire systems may be stored in notebooks and we would not be able to analyze such systems. However, this use case is a bit out-of-scope for our approach as we target industrial DL systems where run-time performance is particularly important. Notebooks are commonly used for prototyping purposes.\addrefRK%

